Saath: Speeding up CoFlows by Exploiting the Spatial Dimension

Coflow scheduling improves data-intensive application performance by improving their networking performance. State-of-the-art Coflow schedulers in essence approximate the classic online Shortest-Job-First (SJF) scheduling, designed for a single CPU, in a distributed setting, with no coordination among how the flows of a Coflow at individual ports are scheduled, and as a result suffer two performance drawbacks: (1) The flows of a Coflow may suffer the out-of-sync problem -- they may be scheduled at different times and become drifting apart, negatively affecting the Coflow completion time (CCT); (2) FIFO scheduling of flows at each port bears no notion of SJF, leading to suboptimal CCT. We propose SAATH, an online Coflow scheduler that overcomes the above drawbacks by explicitly exploiting the spatial dimension of Coflows. In SAATH, the global scheduler schedules the flows of a Coflow using an all-or-none policy which mitigates the out-of-sync problem. To order the Coflows within each queue, SAATH resorts to a Least-Contention-First (LCoF) policy which we show extends the gist of SJF to the spatial dimension, complemented with starvation freedom. Our evaluation using an Azure testbed and simulations of two production cluster traces show that compared to Aalo, SAATH reduces the CCT in median (P90) cases by 1.53x (4.5x) and 1.42x (37x), respectively.

==> outline.tex <==
S1: Intro
S2: Background
    -- 2.1: CoFlow scheduling
    -- 2.2: Aalo design
    -- 2.3: Aalo's limitation: (1) out-of-sync, (2) long delay in determining right queue

S3: Core Ideas
    -- Insight: The key root-cause of the limitations is that Aalo completely missed out the spatial dimension.
    -- 3.1: All-or-none
    -- 3.2: LCoF to reduce average waiting time
    -- 3.3: Per-flow queue thresholds to determine queue faster

S4: Design
    -- 4.1: Architecture (co-ordinator decides the schedule)
    -- 4.2: Scheduling algorithm (main loop for all-or-none, work conservation for rest)
    -- 4.3: Starvation avoidance

S5: Handling cluster dynamics
    -- 5.1: Speeding up CoFlows with skew, failures and stragglers.
            (We move the CoFlows from lower to higher priority queues if they have small set of flows pending)
    -- 5.2: Unavailability of data
    -- 5.3: DAGs and multiple waves

S6: Implementation

S7: Testbed

S8: Simulation

S9: Related Work

S10: Conclusion

Appendix: SJF is not optimal. 


==> related.tex <==
\section{Related Work}
\label{sec:related}

%  There has been
%  much work on CoFlow and job scheduling in general, which we discuss
%  below.

\textbf{Non-Clairvoyant Scheduling}: Non-clairvoyant scheduling, \ie scheduling
without prior knowledge, has been studied as early as in time-sharing
systems~\cite{corbato:1962,coffman:1968}, with many
variations~\cite{nuyens:2008, rai:2003} and applied to diverse scheduling
problems such as memory controller scheduling~\cite{atlas:HPCA2010}.

\textbf{CoFlow scheduling:} 
Varys~\cite{varys:sigcomm14} was proposed
to schedule the CoFlows assuming \textit{prior} information is available.
% which is not practical in online settings. 
In contrast, LCoF is an
online scheduling policy, that in fact performs comparable to offline
SEBF from Varys (Fig.~\ref{fig:sim:cct}). \cite{coflow:spaa15} shows
CoFlow scheduling is NP hard and proposes heuristics to reduce the
average CCT, again assuming prior knowledge of CoFlows. Baraat~\cite{baraat:sigcomm14} and
Aalo~\cite{aalo:sigcomm15} 
schedule CoFlows in online settings.
We have already discussed
Aalo extensively. Baraat is a completely de-centralized scheduler
without coordination among the ports, and suffers
from the same limitation as Aalo. 
%  Graviton~\cite{graviton:hotcloud16}
%  uses width as an indicator to the CoFlow size, and uses different yet
%  \textit{static} scheduling policies in different queues using the
%  width but suffers from the all-or-none problem due to un-coordinated
%  scheduling across its ports. 
In contrast, \name~\cite{jajooSaath} is, to our best knowledge, the first CoFlow
scheduler that takes into consideration the spatial dimension when
scheduling CoFlows, by applying all-or-none and LCoF.
% , and schedules the CoFlows on all the ports using a centralized scheduler.
Recently, CODA~\cite{zhang:sigcomm15} was proposed to automatically
identify flows that belong to the same CoFlows, 
% \ie without modifying data parallel applications,
and schedule them while tolerating identification errors.

\textbf{Flow scheduling:} There has been a rich body of prior work on flow
scheduling. Efforts to minimize FCTs, both with prior information (\eg
PDQ~\cite{pdq:sigcomm12}, pFabric~\cite{pfabric:sigcomm13}) and without prior
information (\eg Fastpass~\cite{fastpass:sigcomm14},
PIAS~\cite{pias:hotnets14}), fall short in minimizing CCTs which depend on the
completion of the last flow~\cite{varys:sigcomm14}. Similarly,
Hedera~\cite{hedera:nsdi10} and MicroTE~\cite{microte:conext11} schedule the
flows with the goal of reducing the overall FCT, which again is different from
reducing the overall CCT of CoFlows. In this~\cite{philaeTechReport,
jajooPhilae} paper authors explore a learning technique for coflows.

\textbf{All-or-none:} The all-or-none principle in \name is also used
in different contexts (\eg caching in Pacman~\cite{pacman:nsdi12}, task placement in
~\cite{allnone:hipc13}). Squall~\cite{allnone:epfl:tech16} uses it to
partition data for scalable and fast query processing.
Fastpass~\cite{fastpass:sigcomm14} uses it to schedule flows in
datacenters.

%\if 0
\textbf{Job scheduling:} There have been much work on scheduling in
analytic systems and storage at scale by improving speculative
tasks~\cite{late:osdi08, mantri:osdi10, dolly:nsdi13, slearnTechReport, jajooSLearn}, improving
locality~\cite{delay:eurosys10, scarlett:eurosys11}, and end-point
flexibility~\cite{sinbad:sigcomm13,rubik:atc15, pisces:osdi12}. The CoFlow
abstraction is complimentary to these work, and can benefit from
them. %% Combining CoFlow with these approaches remains as a future work.
%\fi

\textbf{Scheduling in parallel processors:} CoFlow scheduling by exploiting the
spatial dimension bears similarity to scheduling processes on
parallel processors and multi-cores, where many variations of
FIFO~\cite{cmpproc:soda98}, FIFO with
back-filling~\cite{cmpproc:ipps98} and gang
scheduling~\cite{cmpproc:pp05} are proposed.
% , which are orthogonal to \name.

%% based schedulers are proposed. These
%% schedulers face same problem of low port utilization as not all
%% processors/threads


